Safety-Critical Ergodic Exploration in Cluttered Environments via Control Barrier Functions

In this paper, we address the problem of safe trajectory planning for autonomous search and exploration in constrained, cluttered environments. Guaranteeing safe (collision-free) trajectories is a challenging problem that has garnered significant due to its importance in the successful utilization of robots in search and exploration tasks. This work contributes a method that generates guaranteed safety-critical search trajectories in a cluttered environment. Our approach integrates safety-critical constraints using discrete control barrier functions (DCBFs) with ergodic trajectory optimization to enable safe exploration. Ergodic trajectory optimization plans continuous exploratory trajectories that guarantee complete coverage of a space. We demonstrate through simulated and experimental results on a drone that our approach is able to generate trajectories that enable safe and effective exploration. Furthermore, we show the efficacy of our approach for safe exploration using real-world single- and multi- drone platforms.

==> Ergodic CBF - 2023 ICRA Paper - Final(1)/notepad.tex <==

% Paragraph 1
    % Sentence 1: the use of efficient search algorithms is important to search and rescues operations, robotic exploration, autonomous mapping
    % Sentence 2: we use ergodic search to explore an exploration space.
    % Sentence 3: guaranteeing safe trajectories is important so robots don't collide with other agents or obstacles or themselves
    % Sentence 4: control barrier functions provide us a tool for avoiding obstacles
    % Sentence 5: We show that we can quickly and safely carry out an ergodic search of an exploration space using constraint optimization with control barrier functions to avoid obstacles

% Paragraph 2 (eventually needed, paragraph 1 will be more of an introduction and paragraph 2 will be how we did it)
    % Sentence 1: we use ergodic search 
    % Sentence 2: we introduce the CBF as a constraint during optimization
    % Sentence 3: we are able to quickly and efficiently search an exploration space while avoiding obstacles
    
    
%%%%%%%%%%%%%%%%%%%%%%%%

% What are you doing/motivation.
    %% How do we generate exploration that is safe
    %% methods currently do full coverage but they don't guarantee safety
    %% Used for lots of stuff
    %% Has big impacts in these fields
% Current state of the art methods.
    %% Safety-critical is necessary bc it guarantees safety, especially in cluttered environments.
    %% State of the art safety critical methods (RRT w/ CBF) (but they're not ergodic), reachability analysis (but it scales poorly).
    %% Look at other leading methods for guaranteeing safety
    %% Look at other search methods that do obstacle avoidance
% What is missing.
    %% There are existing methods for planning safety-critical trajectories, but they are not ergodic. There are ergodic methods that plan safe trajectories, but they don't guarantee safety. That's where we come in. 
% What we do
    %% incorporate CBFs into the ergodic search method to generate safety-critical trajectories
% Contributions
    %% safety critical ergodic search trajectory, guaranteeing obstacle avoidance
    %% outperforms other ergodic search w/ basic inequality constraints for obstacle avoidance
    
%%%%%%%%%%%%%%%%%%%%%%%%%
% Contributions
% \IEEEpubidadjcol
% \noindent
% \textbf{Contributions:}
% We show that control barrier functions can be implemented in conjunction with ergodic coverage methods to create safety-critical trajectories in cluttered search environments. Our methods outperform existing state of the art ergodic search methods that avoid obstacles using basic inequality constraints. Through the implementation of CBFs as inequality constraints, we can generate ergodic trajectories that guarantee coverage of an exploration space while avoiding obstacles. These trajectories allow for fast and efficient search of the exploration space and guarantee obstacle avoidance.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                  Related Work                  %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% People use ergodic search for a large number of applications, list several of those applications as they pertain to searching an exploration space and path planning.
% People use CBFs for safety-critical path planning. Touch on some of the ways that they use CBFs as it pertains to path planning. Talk about the CBF/RRT paper that does path planning.

% for each obstacle as an inequality constraint, we can optimize safe trajectories. We then follow these pre-planned trajectories using a quadcopter in both simulation and experiment to conduct a fast, safe, and efficient search of the cluttered exploration space.

Methods that explore while maintaining safety-critical trajectories are desirable because they guarantee obstacle avoidance. 
We implement control barrier functions into ergodic search methods in order to guarantee safety-critical search trajectories. 
Current ergodic search methods (or general search and exploration methods) are capable generating safe trajectories, but these stochastic methods fail to guarantee safety \cite{Salman_Ayvali_Choset_2017}. 
The efficient and safe navigation of autonomous robots address the problem of motion planning for area search/coverage, which arises in many applications such as search and rescue \cite{lee2018receding,liu2013robotic}, environment monitoring \cite {Liu-RSS-19}, target localization \cite{garzon2016multirobot,pimenta2009simultaneous}, self-driving vehicles \cite{}, and autonomous exploration and mapping \cite{}.

% What is missing?
The existing state of the art methods mentioned above that actively explore while guaranteeing safety do not generate ergodic trajectories and therefore lack the accompanying benefits of ergodic coverage. 
The methods that consider frontier detection and reachability analysis also generate safety-critical trajectories but do not scale well and are also not ergodic. 
Path planning methods that utilize vector fields for obstacle avoidance have a drawback of potentially getting stuck in a local minima far away from the goal point \cite{Panagou_2014AvoidanceVectorFields}. 
The existing ergodic coverage methods that plan safe trajectories using stochastic methods by implementing basic inequality constraints and do not guarantee safety. 

% What we do?
We carry out an ergodic search in a cluttered exploration space with numerous static obstacles by treating the path planning as a constrained ergodic trajectory optimization problem. 
We show that by introducing control barrier functions (CBFs) for each obstacle as an inequality constraint, we can optimize safe trajectories. 
We then follow these pre-planned trajectories using a quadcopter in both simulation and experiment to conduct a fast, safe, and efficient search of the cluttered exploration space.

\noindent\textbf{Control Barrier Functions (incomplete)}
Obstacle avoidance in optimization-based control and trajectory planning is needed to ensure that robots can safely navigate during operation. Control Barrier Functions (CBFs) are widely used to enforce the safety-critical constraints on nonlinear systems \cite{Manjuanth_Nguyen_2021SafePlanningCBF}. They have been shown to be an effective way to generate safe trajectories in tight-fitting cluttered environments of polytopes \cite{Thirugnanam_Zeng_Sreenath_2021ObstacleAvoidance}; and have proven to be useful in a wide variety of continuous-time systems (such as precise footstep placement of a high degree of freedom bipedal robots, adaptive cruise control systems, multi-agent systems, and quad-rotor systems \cite{}(multiple citations from agrawal2017discrete) and discrete-time systems\cite{agrawal2017discrete};and for environments with both static and dynamic obstacles \cite{Yang_Vang_Serlin_Belta_Tron_2019MotionPlanningCBF}.  CBFs are characterized by a key property called forward-set invariance which ensures that once an agent enters the safe set, it will no longer be able to leave thereby ensuring its safety \cite{Robey2020LearningCB, WIELAND2007462}.


    % Another method utilizes frontier detection and reachability analysis in a graph-based SLAM method for generating safety-critical search trajectories \cite{Sun_2020FrontierDA}. 
    % Several methods attempt to achieve safety by implementing vector fields surrounding obstacles via either apriori knowledge of the obstacles (more citations here) \cite{Panagou_2014AvoidanceVectorFields} or utilization of sensors such as LiDAR \cite{Schleich_Behnke_2022PotentialFieldAvoidance}. 
    
    % The existing state of the art methods mentioned above that actively explore while guaranteeing safety do not generate ergodic trajectories and therefore lack the accompanying benefits of ergodic coverage. 
    % The methods that consider frontier detection and reachability analysis also generate safety-critical trajectories but do not scale well and are also not ergodic. 
    % Current ergodic search methods (or general search and exploration methods) are capable generating safe trajectories, but these stochastic methods fail to guarantee safety \cite{Salman_Ayvali_Choset_2017_ErgodicObstacles}.
    
        % For safety critical control, we consider a set C, defined as the super-level set of a continuously differentiable function $h: x \in \chi \subset \mathbb{R}^{n}: h(x) \geq 0$.     
        
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% from previous preliminary on ergodic section 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


    % Let $\mathcal{W}=[0,L_1]\times[0,L_2]\times\dots\times[0,L_\nu] \subset \mathbb{R}^\nu$ denote a $\nu$-dimensional search space that is to be explored by a robot.
    % The robot has an $n$-dimensional state space ($n\geq\nu$), and let $q_n:[0,T]\rightarrow\mathbb{R}^n$ denote a trajectory in the state space with $T\in\mathbb{R}^+$ representing the time horizon.
    % The robot (deterministic) dynamics is described as $\dot{q_n}(t)=f(q_n(t),u(t))$, where $u(t)$ is the control input of the robot.
    % Additionally, for each trajectory $q_n$, let $q:[0,T]\rightarrow\mathcal{W}$ denote the corresponding trajectory in the workspace (instead of the state space).

    % Let $c(x,q), x\in\mathcal{W}$ denote the time-averaged statistics of a trajectory $q$, which is defined as:
    % \begin{gather}\label{moes:eqn:time_avg_stat_of_traj}
    %     c(x,q) = \frac{1}{T}\int_{0}^{T} \delta(x-q(\tau))d\tau,
    % \end{gather} where $\delta$ is a Dirac function.
    % Let $\phi:\mathcal{W}\rightarrow\mathbb{R}$ denote a static info map (i.e., a probability distribution), which describes the amount of information at each location in the workspace.
    % An ergodic metric \cite{Mathew_Mezic_2011_Ergodicity} between $c(x,q)$ and an info map $\phi$ is defined as:
    % \begin{equation}
    % \begin{split}
    %     \mathcal{E}(\phi,q) & = \sum_{k=0}^{K}\lambda_k(c_k - \phi_k)^2\\
    %     & =\sum_{k=0}^{K}\lambda_k \left( \frac{1}{T} \int_{0}^{T}F_k(q(\tau))d\tau - \phi_k \right) ^2
    % \end{split}
    % \end{equation}
    % where (i) $\phi_k=\int_{\mathcal{W}}\phi(x)F_k(x)dx$ represents the Fourier coefficients of the info map, with $F_k(q) = \frac{1}{h_k}\Pi_{j=1}^{\nu}\cos(\frac{k_j\pi q_j}{L_j})$ being the cosine basis function for some index $k \in \mathbb{N}^\nu$ and $K$ being the number of Fourier bases considered, (ii) $c_k$ denotes the Fourier coefficient of $c(x,q)$, (iii) $h_k$ denotes the normalization factor as defined in \cite{Mathew_Mezic_2011_Ergodicity}, and (iv) $\lambda_k=(1+||k||^2)^{-\frac{\nu+1}{2}}$ denotes the weight for each corresponding Fourier coefficient.
    
    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    %%%%%%% Below is taken from Thirugnanam_Zeng_Sreenath_2021_ObstacleAvoidance %%%%%%%

    % Obstacle avoidance for safety for this dynamical system is defined in terms of invariance of its trajectories with respect to a connected set \cite{Thirugnanam_Zeng_Sreenath_2021_ObstacleAvoidance}.
    % In other words, if the dynamical system \eqref{eq:dt-system} is safe with respect to a set $\mathcal{S} \subset \mathcal{X}$, then any trajectory starting inside $\mathcal{S}$ remains inside $\mathcal{S}$.
    % The set $\mathcal{S}$ is defined as the 0-superlevel set of a continuous function $h: \mathcal{X} \rightarrow \mathbb{R}$ as:
    % \begin{equation}
    % \label{eq:safe-set-def}
    % \mathcal{S} := \{x \in \mathcal{X} \subset \mathbb{R}^n: h(x) \geq 0\}.
    % \end{equation}
    % We refer to $\mathcal{S}$ as the safe set and it represents the region outside the obstacle. $h$ is defined as a discrete-time control barrier function (DCBF) if $\forall \; x \in \mathcal{S}, \exists \; u \in \mathcal{U}$ such that
    % \begin{equation}
    % \label{eq:dcbf-def}
    % h(f(x_{i,t},u_{i,t})) \geq \gamma(x_{i,t}) h(_x{i,t}), \quad 0 \leq \gamma(x_{i,t}) < 1,
    % \end{equation}
    % Let $\gamma_t := \gamma(x_t)$.
    % Satisfying \eqref{eq:dcbf-def} implies $h(x_{k+1}) \geq \gamma_k h(x_{i,t})$, i.e., the lower bound of the DCBF decreases exponentially with the decay rate $\gamma_k$~\cite{Sreenath_Agrawal_2017_discreteCBF}.
    % Given a choice of $\gamma(x)$, we denote $\mathcal{K}(x)$ as
    % \begin{equation}
    % \label{eq:safe-control-set-def}
    % \mathcal{K}(x) := \{u \in \mathcal{U}: h(f(x,u)) - \gamma(x) h(x) \geq 0\}.
    % \end{equation}
    % Then, if $x_0 \in \mathcal{S}$ and $u_k \in \mathcal{K}(x_k)$, then $x_{k} \in \mathcal{S}$ for $\forall \; k \in \mathbb{Z}^+$, i.e., the resulting trajectory is safe~\cite{Sreenath_Agrawal_2017_discreteCBF}.

    % Given a valid DCBF $h$~\cite{Ames_Sreenath_Egerstedt_Tabuada_2019_CBFTheoryandApp}, imposing DCBF constraint \eqref{eq:dcbf-def} in an optimization problem could guarantee system safety, i.e., collision-free trajectories.
    % If $\gamma(x)$ is close to $1$, the system converges to $\partial \mathcal{S}$ slowly but can easily become infeasible."
    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    Ergodic theory is the study of the long-term average behaviour of dynamical systems \cite{Petersen_1983_IntroductionErgodicTheory}. 
    In robotic search and exploration, ergodic trajectory optimization computes control laws that drive a dynamic system along trajectories such that the amount of time spent in regions of the state space is proportional to the expected information gain in those regions \cite{Miller_Murphy_2016_ErgodicExploration}.
    
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        % metric in Eq.~\ref{eq:ergodic_disc} and DCBF in Eq.~\ref{eq:dcbf-def} into the following constrained ergodic trajectory optimization problem:
    % \noindent\rule{\columnwidth}{0.4pt}
    % \textbf{Safety-Critical Ergodic Trajectory Optimization:}
    % \begin{subequations}\label{eq:ergodic-opt}
    % \begin{align}
    %     J_{t}^{*}(\mathbf{x}_t,\mathbf{u}_t) =  \min_{\mathbf{x}, \mathbf{u}} p(\mathbf{x}_{t+N|t}){+}\sum_{k=0}^{N-1} & q(\mathbf{x}_{t+k|t},\mathbf{u}_{t+k|t}) \label{eq:mpc-cost}\\
    %     \text{s.t.} \quad 
    %     \mathbf{x}_{t+k+1|t} = f(\mathbf{x}_{t+k|t}, \mathbf{u}_{t+k|t}), & \ k = 0,...,N{-}1  \label{eq:mpc-system-dynamics}\\
    %     \mathbf{x}_{t+k|t} \in \mathcal{X}, \mathbf{u}_{t+k|t} \in \mathcal{U}, & \ k = 0,...,N{-}1 \label{eq:mpc-state-input-constraint}\\
    %     \mathbf{x}_{t|t} = \mathbf{x}_t, \label{eq:mpc-current-state} \\
    %     \mathbf{x}_{t+N|t} \in \mathcal{X}_f, & \label{eq:mpc-terminal-set}\\
    %     g(\mathbf{x}_{t+k|t}) \geq 0, &\ k = 0,...,N{-}1. \label{eq:mpc-distance-constraint}
    % \end{align}
    % \end{subequations}
    % \noindent\rule{\columnwidth}{0.4pt}
    % We use the method of Augmented Lagrange Multipliers to solve the optimization problem, which jointly optimizes the states and controls using collocation methods. 
    
    % Our cluttered exploration space contains an assortment of obstacles that vary in size, shape, and orientation and implementing the DCBF as an inequality constraint allows us to build a safety barrier around each obstacle (Fig. ~\ref{fig++}). 
    % Using simulations and experiments we show that we can safely and efficiently search the exploration space (Figs.~\ref{fig1},\ref{fig_num}). 
    

% • Pre-planned path for the quadrotor to follow (fig 1)
% • Statistics for how tuning different control parameters effect whether or not it hits an obstacle.
% • statistics for the collision rate for different initial conditions
% • collision statistics for using the CBF constraint vs just a distance cutoff constraint (loose)
    
    
    % \section{Appendix}\label{sec:appendix}
        % We use the following exponential discrete CBF: 
    % \begin{equation}
    % \begin{split}
    % \label{eq:cbf}
    % h(x_{i,t}, y_{i,t}) = 1 - \left(\frac{x_{i,t} - x_{obstacle}}{R_{y max}}\right)^{a} - \left(\frac{y_{i,t} - y_{obstacle}}{R_{x max}}\right)^{b}
    % \end{split}
    % \end{equation}
    % where $(x_{i,t},y_{i,t})$ is the position of agent $i$ at time $t$, the center of each obstacle is represented by $x,y_{obstacle}$, and $R_{x,y max}$ is the size of the barrier.  The shape of the barrier can be tuned from a squared-ellipse ($a,b=4$) to a circle squared-ellipse ($a,b=2$).
    
        % Given a choice of $\gamma$, we denote $\mathcal{K}(x)$ as
    % \begin{equation}
    % \label{eq:safe-control-set-def}
    % \mathcal{K}(x) := \{u \in \mathcal{U}: h(f(x,u)) - \gamma h(x) \geq 0\}.
    % \end{equation}
    % Then, if $x_0 \in \mathcal{S}$ and $u_k \in \mathcal{K}(x)$, then $x_{t} \in \mathcal{S}$, $\forall t$, i.e., the resulting trajectory is safe~\cite{Sreenath_Agrawal_2017_discreteCBF}.

==> Ergodic CBF - 2023 ICRA Paper - Final(1)/video_summary.tex <==
Title: 'Safety-Critical Ergodic Exploration in Cluttered Environments via
Control Barrier Functions'

Authors: Cameron Lerch, Ethan Dong, and Ian Abraham

Video Category: Regular Video

Abstract:
We address the problem of safe trajectory planning for autonomous search and exploration in constrained, cluttered environments. Guaranteeing safe navigation is a challenging problem that has garnered significant attention. This work contributes a method that generates guaranteed safety-critical search trajectories in a cluttered environment. Our approach integrates safety-critical constraints using discrete control barrier functions (DCBFs) with ergodic trajectory optimization to enable safe exploration. Ergodic trajectory optimization plans continuous exploratory trajectories that guarantee full coverage of a space. We demonstrate through simulated and experimental results on a drone that
our approach is able to generate trajectories that enable safe and effective exploration. Furthermore, we show the efficacy of our approach for safe exploration of real-world single- and
multi- drone platforms.

Contact Information:
Name:   Cameron Lerch
email:  cameron.lerch@gmail.com

Name:   Ethan Dong
email:  ethan.dong@yale.edu

Name:   Ian Abraham
email:  ian.abraham@yale.edu

==> notepad.tex <==

% Paragraph 1
    % Sentence 1: the use of efficient search algorithms is important to search and rescues operations, robotic exploration, autonomous mapping
    % Sentence 2: we use ergodic search to explore an exploration space.
    % Sentence 3: guaranteeing safe trajectories is important so robots don't collide with other agents or obstacles or themselves
    % Sentence 4: control barrier functions provide us a tool for avoiding obstacles
    % Sentence 5: We show that we can quickly and safely carry out an ergodic search of an exploration space using constraint optimization with control barrier functions to avoid obstacles

% Paragraph 2 (eventually needed, paragraph 1 will be more of an introduction and paragraph 2 will be how we did it)
    % Sentence 1: we use ergodic search 
    % Sentence 2: we introduce the CBF as a constraint during optimization
    % Sentence 3: we are able to quickly and efficiently search an exploration space while avoiding obstacles
    
    
%%%%%%%%%%%%%%%%%%%%%%%%

% What are you doing/motivation.
    %% How do we generate exploration that is safe
    %% methods currently do full coverage but they don't guarantee safety
    %% Used for lots of stuff
    %% Has big impacts in these fields
% Current state of the art methods.
    %% Safety-critical is necessary bc it guarantees safety, especially in cluttered environments.
    %% State of the art safety critical methods (RRT w/ CBF) (but they're not ergodic), reachability analysis (but it scales poorly).
    %% Look at other leading methods for guaranteeing safety
    %% Look at other search methods that do obstacle avoidance
% What is missing.
    %% There are existing methods for planning safety-critical trajectories, but they are not ergodic. There are ergodic methods that plan safe trajectories, but they don't guarantee safety. That's where we come in. 
% What we do
    %% incorporate CBFs into the ergodic search method to generate safety-critical trajectories
% Contributions
    %% safety critical ergodic search trajectory, guaranteeing obstacle avoidance
    %% outperforms other ergodic search w/ basic inequality constraints for obstacle avoidance
    
%%%%%%%%%%%%%%%%%%%%%%%%%
% Contributions
% \IEEEpubidadjcol
% \noindent
% \textbf{Contributions:}
% We show that control barrier functions can be implemented in conjunction with ergodic coverage methods to create safety-critical trajectories in cluttered search environments. Our methods outperform existing state of the art ergodic search methods that avoid obstacles using basic inequality constraints. Through the implementation of CBFs as inequality constraints, we can generate ergodic trajectories that guarantee coverage of an exploration space while avoiding obstacles. These trajectories allow for fast and efficient search of the exploration space and guarantee obstacle avoidance.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                  Related Work                  %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% People use ergodic search for a large number of applications, list several of those applications as they pertain to searching an exploration space and path planning.
% People use CBFs for safety-critical path planning. Touch on some of the ways that they use CBFs as it pertains to path planning. Talk about the CBF/RRT paper that does path planning.

% for each obstacle as an inequality constraint, we can optimize safe trajectories. We then follow these pre-planned trajectories using a quadcopter in both simulation and experiment to conduct a fast, safe, and efficient search of the cluttered exploration space.

Methods that explore while maintaining safety-critical trajectories are desirable because they guarantee obstacle avoidance. 
We implement control barrier functions into ergodic search methods in order to guarantee safety-critical search trajectories. 
Current ergodic search methods (or general search and exploration methods) are capable generating safe trajectories, but these stochastic methods fail to guarantee safety \cite{Salman_Ayvali_Choset_2017}. 
The efficient and safe navigation of autonomous robots address the problem of motion planning for area search/coverage, which arises in many applications such as search and rescue \cite{lee2018receding,liu2013robotic}, environment monitoring \cite {Liu-RSS-19}, target localization \cite{garzon2016multirobot,pimenta2009simultaneous}, self-driving vehicles \cite{}, and autonomous exploration and mapping \cite{}.

% What is missing?
The existing state of the art methods mentioned above that actively explore while guaranteeing safety do not generate ergodic trajectories and therefore lack the accompanying benefits of ergodic coverage. 
The methods that consider frontier detection and reachability analysis also generate safety-critical trajectories but do not scale well and are also not ergodic. 
Path planning methods that utilize vector fields for obstacle avoidance have a drawback of potentially getting stuck in a local minima far away from the goal point \cite{Panagou_2014AvoidanceVectorFields}. 
The existing ergodic coverage methods that plan safe trajectories using stochastic methods by implementing basic inequality constraints and do not guarantee safety. 

% What we do?
We carry out an ergodic search in a cluttered exploration space with numerous static obstacles by treating the path planning as a constrained ergodic trajectory optimization problem. 
We show that by introducing control barrier functions (CBFs) for each obstacle as an inequality constraint, we can optimize safe trajectories. 
We then follow these pre-planned trajectories using a quadcopter in both simulation and experiment to conduct a fast, safe, and efficient search of the cluttered exploration space.

\noindent\textbf{Control Barrier Functions (incomplete)}
Obstacle avoidance in optimization-based control and trajectory planning is needed to ensure that robots can safely navigate during operation. Control Barrier Functions (CBFs) are widely used to enforce the safety-critical constraints on nonlinear systems \cite{Manjuanth_Nguyen_2021SafePlanningCBF}. They have been shown to be an effective way to generate safe trajectories in tight-fitting cluttered environments of polytopes \cite{Thirugnanam_Zeng_Sreenath_2021ObstacleAvoidance}; and have proven to be useful in a wide variety of continuous-time systems (such as precise footstep placement of a high degree of freedom bipedal robots, adaptive cruise control systems, multi-agent systems, and quad-rotor systems \cite{}(multiple citations from agrawal2017discrete) and discrete-time systems\cite{agrawal2017discrete};and for environments with both static and dynamic obstacles \cite{Yang_Vang_Serlin_Belta_Tron_2019MotionPlanningCBF}.  CBFs are characterized by a key property called forward-set invariance which ensures that once an agent enters the safe set, it will no longer be able to leave thereby ensuring its safety \cite{Robey2020LearningCB, WIELAND2007462}.


    % Another method utilizes frontier detection and reachability analysis in a graph-based SLAM method for generating safety-critical search trajectories \cite{Sun_2020FrontierDA}. 
    % Several methods attempt to achieve safety by implementing vector fields surrounding obstacles via either apriori knowledge of the obstacles (more citations here) \cite{Panagou_2014AvoidanceVectorFields} or utilization of sensors such as LiDAR \cite{Schleich_Behnke_2022PotentialFieldAvoidance}. 
    
    % The existing state of the art methods mentioned above that actively explore while guaranteeing safety do not generate ergodic trajectories and therefore lack the accompanying benefits of ergodic coverage. 
    % The methods that consider frontier detection and reachability analysis also generate safety-critical trajectories but do not scale well and are also not ergodic. 
    % Current ergodic search methods (or general search and exploration methods) are capable generating safe trajectories, but these stochastic methods fail to guarantee safety \cite{Salman_Ayvali_Choset_2017_ErgodicObstacles}.
    
        % For safety critical control, we consider a set C, defined as the super-level set of a continuously differentiable function $h: x \in \chi \subset \mathbb{R}^{n}: h(x) \geq 0$.     
        
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% from previous preliminary on ergodic section 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


    % Let $\mathcal{W}=[0,L_1]\times[0,L_2]\times\dots\times[0,L_\nu] \subset \mathbb{R}^\nu$ denote a $\nu$-dimensional search space that is to be explored by a robot.
    % The robot has an $n$-dimensional state space ($n\geq\nu$), and let $q_n:[0,T]\rightarrow\mathbb{R}^n$ denote a trajectory in the state space with $T\in\mathbb{R}^+$ representing the time horizon.
    % The robot (deterministic) dynamics is described as $\dot{q_n}(t)=f(q_n(t),u(t))$, where $u(t)$ is the control input of the robot.
    % Additionally, for each trajectory $q_n$, let $q:[0,T]\rightarrow\mathcal{W}$ denote the corresponding trajectory in the workspace (instead of the state space).

    % Let $c(x,q), x\in\mathcal{W}$ denote the time-averaged statistics of a trajectory $q$, which is defined as:
    % \begin{gather}\label{moes:eqn:time_avg_stat_of_traj}
    %     c(x,q) = \frac{1}{T}\int_{0}^{T} \delta(x-q(\tau))d\tau,
    % \end{gather} where $\delta$ is a Dirac function.
    % Let $\phi:\mathcal{W}\rightarrow\mathbb{R}$ denote a static info map (i.e., a probability distribution), which describes the amount of information at each location in the workspace.
    % An ergodic metric \cite{Mathew_Mezic_2011_Ergodicity} between $c(x,q)$ and an info map $\phi$ is defined as:
    % \begin{equation}
    % \begin{split}
    %     \mathcal{E}(\phi,q) & = \sum_{k=0}^{K}\lambda_k(c_k - \phi_k)^2\\
    %     & =\sum_{k=0}^{K}\lambda_k \left( \frac{1}{T} \int_{0}^{T}F_k(q(\tau))d\tau - \phi_k \right) ^2
    % \end{split}
    % \end{equation}
    % where (i) $\phi_k=\int_{\mathcal{W}}\phi(x)F_k(x)dx$ represents the Fourier coefficients of the info map, with $F_k(q) = \frac{1}{h_k}\Pi_{j=1}^{\nu}\cos(\frac{k_j\pi q_j}{L_j})$ being the cosine basis function for some index $k \in \mathbb{N}^\nu$ and $K$ being the number of Fourier bases considered, (ii) $c_k$ denotes the Fourier coefficient of $c(x,q)$, (iii) $h_k$ denotes the normalization factor as defined in \cite{Mathew_Mezic_2011_Ergodicity}, and (iv) $\lambda_k=(1+||k||^2)^{-\frac{\nu+1}{2}}$ denotes the weight for each corresponding Fourier coefficient.
    
    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    %%%%%%% Below is taken from Thirugnanam_Zeng_Sreenath_2021_ObstacleAvoidance %%%%%%%

    % Obstacle avoidance for safety for this dynamical system is defined in terms of invariance of its trajectories with respect to a connected set \cite{Thirugnanam_Zeng_Sreenath_2021_ObstacleAvoidance}.
    % In other words, if the dynamical system \eqref{eq:dt-system} is safe with respect to a set $\mathcal{S} \subset \mathcal{X}$, then any trajectory starting inside $\mathcal{S}$ remains inside $\mathcal{S}$.
    % The set $\mathcal{S}$ is defined as the 0-superlevel set of a continuous function $h: \mathcal{X} \rightarrow \mathbb{R}$ as:
    % \begin{equation}
    % \label{eq:safe-set-def}
    % \mathcal{S} := \{x \in \mathcal{X} \subset \mathbb{R}^n: h(x) \geq 0\}.
    % \end{equation}
    % We refer to $\mathcal{S}$ as the safe set and it represents the region outside the obstacle. $h$ is defined as a discrete-time control barrier function (DCBF) if $\forall \; x \in \mathcal{S}, \exists \; u \in \mathcal{U}$ such that
    % \begin{equation}
    % \label{eq:dcbf-def}
    % h(f(x_{i,t},u_{i,t})) \geq \gamma(x_{i,t}) h(_x{i,t}), \quad 0 \leq \gamma(x_{i,t}) < 1,
    % \end{equation}
    % Let $\gamma_t := \gamma(x_t)$.
    % Satisfying \eqref{eq:dcbf-def} implies $h(x_{k+1}) \geq \gamma_k h(x_{i,t})$, i.e., the lower bound of the DCBF decreases exponentially with the decay rate $\gamma_k$~\cite{Sreenath_Agrawal_2017_discreteCBF}.
    % Given a choice of $\gamma(x)$, we denote $\mathcal{K}(x)$ as
    % \begin{equation}
    % \label{eq:safe-control-set-def}
    % \mathcal{K}(x) := \{u \in \mathcal{U}: h(f(x,u)) - \gamma(x) h(x) \geq 0\}.
    % \end{equation}
    % Then, if $x_0 \in \mathcal{S}$ and $u_k \in \mathcal{K}(x_k)$, then $x_{k} \in \mathcal{S}$ for $\forall \; k \in \mathbb{Z}^+$, i.e., the resulting trajectory is safe~\cite{Sreenath_Agrawal_2017_discreteCBF}.

    % Given a valid DCBF $h$~\cite{Ames_Sreenath_Egerstedt_Tabuada_2019_CBFTheoryandApp}, imposing DCBF constraint \eqref{eq:dcbf-def} in an optimization problem could guarantee system safety, i.e., collision-free trajectories.
    % If $\gamma(x)$ is close to $1$, the system converges to $\partial \mathcal{S}$ slowly but can easily become infeasible."
    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    Ergodic theory is the study of the long-term average behaviour of dynamical systems \cite{Petersen_1983_IntroductionErgodicTheory}. 
    In robotic search and exploration, ergodic trajectory optimization computes control laws that drive a dynamic system along trajectories such that the amount of time spent in regions of the state space is proportional to the expected information gain in those regions \cite{Miller_Murphy_2016_ErgodicExploration}.
    
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
        % metric in Eq.~\ref{eq:ergodic_disc} and DCBF in Eq.~\ref{eq:dcbf-def} into the following constrained ergodic trajectory optimization problem:
    % \noindent\rule{\columnwidth}{0.4pt}
    % \textbf{Safety-Critical Ergodic Trajectory Optimization:}
    % \begin{subequations}\label{eq:ergodic-opt}
    % \begin{align}
    %     J_{t}^{*}(\mathbf{x}_t,\mathbf{u}_t) =  \min_{\mathbf{x}, \mathbf{u}} p(\mathbf{x}_{t+N|t}){+}\sum_{k=0}^{N-1} & q(\mathbf{x}_{t+k|t},\mathbf{u}_{t+k|t}) \label{eq:mpc-cost}\\
    %     \text{s.t.} \quad 
    %     \mathbf{x}_{t+k+1|t} = f(\mathbf{x}_{t+k|t}, \mathbf{u}_{t+k|t}), & \ k = 0,...,N{-}1  \label{eq:mpc-system-dynamics}\\
    %     \mathbf{x}_{t+k|t} \in \mathcal{X}, \mathbf{u}_{t+k|t} \in \mathcal{U}, & \ k = 0,...,N{-}1 \label{eq:mpc-state-input-constraint}\\
    %     \mathbf{x}_{t|t} = \mathbf{x}_t, \label{eq:mpc-current-state} \\
    %     \mathbf{x}_{t+N|t} \in \mathcal{X}_f, & \label{eq:mpc-terminal-set}\\
    %     g(\mathbf{x}_{t+k|t}) \geq 0, &\ k = 0,...,N{-}1. \label{eq:mpc-distance-constraint}
    % \end{align}
    % \end{subequations}
    % \noindent\rule{\columnwidth}{0.4pt}
    % We use the method of Augmented Lagrange Multipliers to solve the optimization problem, which jointly optimizes the states and controls using collocation methods. 
    
    % Our cluttered exploration space contains an assortment of obstacles that vary in size, shape, and orientation and implementing the DCBF as an inequality constraint allows us to build a safety barrier around each obstacle (Fig. ~\ref{fig++}). 
    % Using simulations and experiments we show that we can safely and efficiently search the exploration space (Figs.~\ref{fig1},\ref{fig_num}). 
    

% • Pre-planned path for the quadrotor to follow (fig 1)
% • Statistics for how tuning different control parameters effect whether or not it hits an obstacle.
% • statistics for the collision rate for different initial conditions
% • collision statistics for using the CBF constraint vs just a distance cutoff constraint (loose)
    
    
    % \section{Appendix}\label{sec:appendix}
        % We use the following exponential discrete CBF: 
    % \begin{equation}
    % \begin{split}
    % \label{eq:cbf}
    % h(x_{i,t}, y_{i,t}) = 1 - \left(\frac{x_{i,t} - x_{obstacle}}{R_{y max}}\right)^{a} - \left(\frac{y_{i,t} - y_{obstacle}}{R_{x max}}\right)^{b}
    % \end{split}
    % \end{equation}
    % where $(x_{i,t},y_{i,t})$ is the position of agent $i$ at time $t$, the center of each obstacle is represented by $x,y_{obstacle}$, and $R_{x,y max}$ is the size of the barrier.  The shape of the barrier can be tuned from a squared-ellipse ($a,b=4$) to a circle squared-ellipse ($a,b=2$).
    
        % Given a choice of $\gamma$, we denote $\mathcal{K}(x)$ as
    % \begin{equation}
    % \label{eq:safe-control-set-def}
    % \mathcal{K}(x) := \{u \in \mathcal{U}: h(f(x,u)) - \gamma h(x) \geq 0\}.
    % \end{equation}
    % Then, if $x_0 \in \mathcal{S}$ and $u_k \in \mathcal{K}(x)$, then $x_{t} \in \mathcal{S}$, $\forall t$, i.e., the resulting trajectory is safe~\cite{Sreenath_Agrawal_2017_discreteCBF}.

==> video_summary.tex <==
Title: 'Safety-Critical Ergodic Exploration in Cluttered Environments via
Control Barrier Functions'

Authors: Cameron Lerch, Ethan Dong, and Ian Abraham

Video Category: Regular Video

Abstract:
We address the problem of safe trajectory planning for autonomous search and exploration in constrained, cluttered environments. Guaranteeing safe navigation is a challenging problem that has garnered significant attention. This work contributes a method that generates guaranteed safety-critical search trajectories in a cluttered environment. Our approach integrates safety-critical constraints using discrete control barrier functions (DCBFs) with ergodic trajectory optimization to enable safe exploration. Ergodic trajectory optimization plans continuous exploratory trajectories that guarantee full coverage of a space. We demonstrate through simulated and experimental results on a drone that
our approach is able to generate trajectories that enable safe and effective exploration. Furthermore, we show the efficacy of our approach for safe exploration of real-world single- and
multi- drone platforms.

Contact Information:
Name:   Cameron Lerch
email:  cameron.lerch@gmail.com

Name:   Ethan Dong
email:  ethan.dong@yale.edu

Name:   Ian Abraham
email:  ian.abraham@yale.edu
